Statistical Mechanics of Neural Processing of Object Manifolds

Invariant object recognition is one of the most fundamental cognitive tasks performed by the brain. In the neural state space, different objects with stimulus variabilities are represented as different manifolds. In this geometrical perspective, object recognition becomes the problem of linearly separating different object manifolds. In feedforward visual hierarchy, it has been suggested that the object manifold representations are reformatted across the layers, to become more linearly separable. Thus, a complete theory of perception requires characterizing the ability of linear readout networks to classify object manifolds from variable neural responses. A theory of the perceptron of isolated points was pioneered by E. Gardner who formulated it as a statistical mechanics problem and analyzed it using replica theory. In this thesis, we generalize Gardner's analysis and establish a theory of linear classification of manifolds synthesizing statistical and geometric properties of high dimensional signals. [..] Next, we generalize our theory further to linear classification of general perceptual manifolds, such as point clouds. We identify that the capacity of a manifold is determined that effective radius, R_M, and effective dimension, D_M. Finally, we show extensions relevant for applications to real data, incorporating correlated manifolds, heterogenous manifold geometries, sparse labels and nonlinear classifications. Then, we demonstrate how object-based manifolds transform in standard deep networks. This thesis lays the groundwork for a computational theory of neuronal processing of objects, providing quantitative measures for linear separability of object manifolds. We hope this theory will provide new insights into the computational principles underlying processing of sensory representations in biological and artificial neural networks.

==> endmatter/colophon.tex <==
%!TEX root = ../dissertation.tex
\newpage

% If you do want an image in the colophon:
\begin{figure}
  \vspace{20pt}
  \centering
  \hspace*{-32pt}
  \includegraphics[width=0.42\textwidth]{endmatter/colophon.png}
\end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{200pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface. The above illustration, \textit{Science Experiment 02}, was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}. A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.}
\end{center}


==> endmatter/personalize.tex <==
%!TEX root = ../dissertation.tex


==> frontmatter/abstract.tex <==
%!TEX root = ../dissertation.tex
% the abstract

Invariant object recognition is one of the most fundamental cognitive
tasks performed by the brain. In the neural state space, different
objects with stimulus variabilities are represented as different manifolds.
In this geometrical perspective, object recognition becomes the problem
of linearly separating different object manifolds. In feedforward
visual hierarchy, it has been suggested that the object manifold representations
are reformatted across the layers, to become more linearly separable.
Thus, a complete theory of perception requires characterizing the
ability of linear readout networks to classify object manifolds from
variable neural responses. 

A theoretical understanding of the perceptron of isolated points was
pioneered by Elizabeth Gardner who formulated it as a statistical
mechanics problem and analyzed it using replica theory. In this thesis,
we generalize the statistical mechanical analysis and establish a
theory of linear classification of manifolds synthesizing statistical
and geometric properties of high dimensional signals. 

First, we study the theory of linear classification of simple spherical
manifolds, such as line segments, $L_{2}$ balls, or $L_{1}$ balls.
We provide analytical formula for classification capacity of balls,
as a function of dimension, radius, and margin. We also find that
the notion of support vectors needs to be generalized, and identify
different support configurations of the manifolds, which has implications
in generalization error. 

Next, we present a Maximum Margin Manifold Machine ($M_{4}$), an
efficient iterative algorithm that can find a maximum margin linear
binary classifier for manifolds with an uncountable set of training
samples per each manifold. We provide a convergence proof with a polynomial
bound on the convergence time. We further generalize $M_{4}$ for
non-separable manifolds with slack variables. We report that the number
of training examples required to achieve the same generalization error
is much smaller for $M_{4}$, compared with traditional support vector
machines. 

Next, we generalize our theory further to linear classification of
random general manifolds. We start with classification capacity of
random ellipsoids, and generalize to classification capacity of general
smooth and non-smooth manifolds. We identify that the capacity of
a manifold is determined that effective radius, $R_{M}$, and effective
dimension, $D_{M}$. 

Finally, we show extensions to directions relevant for applications to real data. We have extended our general manifold classification theory to incorporate correlated manifolds, mixtures of manifold geometries, sparse labels and nonlinear classifications. Then, we analyze how object-based manifolds reformat in a conventional deep network (GoogLeNet). We find that the deep network indeed changes the manifolds in the direction that the capacity is increased.  

This thesis lays the groundwork for a computational theory of neuronal processing of objects, providing quantitative measures for linear separability of object manifolds. We hope that our theory will provide new insights into the computational principles underlying processing of sensory representations in the brain. As manifold representations of the sensory world are ubiquitous in both biological and artificial neural systems, exciting future work lies ahead. 




==> frontmatter/authorlist.tex <==
%!TEX root = ../dissertation.tex
\noindent Chapter 2 appeared in Physical Review E as: 


Chung, SueYeon, Daniel D. Lee, and Haim Sompolinsky. ``Linear
readout of object manifolds." Physical Review E 93.6
(2016): 060301.\\


\noindent Chapter 3 has been submitted for peer review as: 


Chung, SueYeon, Uri Cohen, Haim Sompolinsky, and Daniel D. Lee. ``The
Maximum Margin Manifold Machine: Efficient Learning with Uncountable
Sets of Training Examples" \\


\noindent An edited version of Chapters 4 will be submitted for a peer
reviewed journal under the title: 


Chung, SueYeon, Daniel D. Lee and Haim Sompolinsky. ``Neural Processing
of Object Manifolds'' \\


\noindent Chapter 5 contains contributions from Daniel D. Lee and Haim Sompolinsky. 


==> frontmatter/junk/dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text

%To Dilu, Mami, Tati, and Delaney. 

%And to Bianca -- the best friendships are forever.

To my parents. 

==> frontmatter/personalize.tex <==
%!TEX root = ../dissertation.tex
% Some details about the dissertation.
\title{Statistical Mechanics of \\Neural Processing of Object Manifolds}
\author{SueYeon Chung}

%If you have one advisor
%\advisor{Haim Sompolinsky}
%If you are coadvised
\coadvisorOne{Haim Sompolinsky}
%\coadvisorTwo{Ryan P. Adams}

\committeeInternalOne{Ryan P. Adams (SEAS co-advisor)}
\committeeInternalTwo{Leslie Valiant}
\committeeInternalThree{David Cox}

%\committeeInternal{Person Inside}

% Everyone has an External committee member
%\committeeExternal{Person Outside}

% ... about the degree.
\degree{Doctor of Philosophy}
\field{Applied Physics}
\degreeyear{2017}
\degreeterm{Spring}
\degreemonth{April}
\department{Engineering and Applied Sciences}

% ... about the candidate's previous degrees.
\pdOneName{B.A.}
\pdOneSchool{Cornell University}
\pdOneYear{2009}


==> frontmatter/thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

This thesis is a testament of the immense amount of support I received from my advisors, mentors, friends, and family throughout the graduate school. 

I have been extremely fortunate to have Haim Sompolinsky as my dissertation advisor, or more suitably, an academic father. Learning from Haim during the formative years of my academic career was one of the best things that have happened in my life. I am deeply indebted to Haim, for generously sharing his knowledge, ideas, feedback and time with me, and teaching me by example how to pick and ask interesting scientific questions and turning them into solvable ones. Most importantly, I am thankful to Haim for showing me the joy and fun in life dedicated to science.  

I am also deeply thankful to Daniel D. Lee, whom I had an honor to work with, on most of the work presented in this thesis. I have learned a lot about formulating a problem into a mathematically attackable one by seeing how Dan does it elegantly. Dan has also been very generous with his help and suggestions -- I am grateful for his warm mentorship and guidance.  

I would like to thank Ryan Adams, my SEAS co-advisor, whose support has been vital for my graduate work at Harvard. I took my first machine learning class with Ryan, whose passion for the study of intelligent systems was an inspiration. I have also learned a lot by attending his group meetings and discussing ideas with him and his group members. I am thankful to Ryan for generous sharing of his time, feedback and advice. 

I would also like to thank the members of my thesis committee, Les Valiant and David Cox, whose guidance and advice have been invaluable. Their generous sharing of time and ideas have had an important impact on the direction and perspective of my research. 

I would like to also thank Yoram Burak, with whom I have worked on the first project in graduate school on perceptual invariance as optimal decoding with neural noise, got me thinking about invariance. I would also like to thank Uri Cohen, with whom I had many valuable discussions on perceptual invariance. I have learned a lot from these collaborations. 

I am indebted to the members of Sompolinsky lab and Center for Brain Science. I am grateful to Ran Rubin, Baktash Babadi, Cengiz Pehlevan, Julijana Gjorgjieva, James Fitzgerald, Yu Hu, Andrew Saxe, Madhu Advani, Dyuti Bhattacharya, Jonathan Kadmon, Itamar Landau, Gadi Mintz, Ariel Furstenberg for many discussions, feedback and encouragement. Many of them were my teachers and also great friends, and it has been a pleasure and privilege to be part of such an inspiring and supportive group. 

I also thank Kenneth Blum, Grace Cho from CBS and Irit Dagan from Hebrew University. I also thank administrators at Harvard SEAS, GSAS and HIO for providing an essential support for my graduate work at Harvard. 

I thank my friends at Harvard and elsewhere -- Seongmin, Jean, Jeongmo, Jake Lee, Soomin, Sunha -- for their support, encouragement and friendship. I am also grateful to my friends in Israel -- Siwei, Neta, and Merav -- for their caring friendship and making Jerusalem another home. 

I am particularly thankful to Jo for always challenging me to be a better version of myself, through the continued support and encouragement, and sharing the great adventure of graduate school. 

I am indebted to my parents, Youngmi and Oonjoo, who have always encouraged me to pursue my dream. I am deeply grateful for the opportunities they have given me. I am also thankful to my siblings, HaeYeon and Yunsoo, for being the best friends and cohort for life. I am forever grateful for my family's unwavering love, support and encouragement. 


